LeForecast: Enterprise Hybrid Forecast by Time Series Intelligence

Demand is spiking in industrial fields for multidisciplinary forecasting, where a broad spectrum of sectors needs planning and forecasts to streamline intelligent business management, such as demand forecasting, product planning, inventory optimization, etc. Specifically, these tasks expecting intelligent approaches to learn from sequentially collected historical data and then foresee most possible trend, i.e. time series forecasting. Challenge of it lies in interpreting complex business contexts and the efficiency and generalisation of modelling. With aspirations of pre-trained foundational models for such purpose, given their remarkable success of large foundation model across legions of tasks, we disseminate \leforecast{}, an enterprise intelligence platform tailored for time series tasks. It integrates advanced interpretations of time series data and multi-source information, and a three-pillar modelling engine combining a large foundation model (Le-TSFM), multimodal model and hybrid model to derive insights, predict or infer futures, and then drive optimisation across multiple sectors in enterprise operations. The framework is composed by a model pool, model profiling module, and two different fusion approaches regarding original model architectures. Experimental results verify the efficiency of our trail fusion concepts: router-based fusion network and coordination of large and small models, resulting in high costs for redundant development and maintenance of models. This work reviews deployment of LeForecast and its performance in three industrial use cases. Our comprehensive experiments indicate that LeForecast is a profound and practical platform for efficient and competitive performance. And we do hope that this work can enlighten the research and grounding of time series techniques in accelerating enterprise.

==> Makefile <==
BASE=template
DIRECTORY=HYPERRIDEDeliverable
bib:
	bibtool  -v -d -s -- 'preserve.key.case=on' -x $(BASE).aux > $(BASE)-new.bib
	mv $(BASE).bib	$(BASE)-old.bib	
	mv $(BASE)-new.bib $(BASE).bib

#dist: bib
dist:
	cd .. && tar hcfvz /tmp/$(DIRECTORY).tgz --exclude-from=$(DIRECTORY)/exclude.txt $(DIRECTORY)/ 

zip:
	cd .. && zip -r /tmp/$(DIRECTORY) $(DIRECTORY)/ -x@$(DIRECTORY)/exclude.txt 

distzip: bib zip

diffpdf:
	latexdiff-vc --git -r $(BASE).tex --pdf 
	-rm $(BASE)-diff.aux 
	-rm $(BASE)-diff.log
	-rm $(BASE)-diff.blg
	-rm $(BASE)-diff.bbl

## NB: please make sure a tag to the submitted version has been added. E.g.:
##
##     git tag -a submitted de73354f15603ceef470eebb3cac28f16ba014fd
##
diffsubmitted: ARGS=submitted
diffsubmitted: diffversion
	@echo Generated diff between the current and submitted versions $(BASE)-diff${ARGS}.pdf

## run as, for instance:
##      make ARGS=de73354f15603ceef470eebb3cac28f16ba014fd diffversion
##
diffversion:
	mkdir -p /tmp/${ARGS}
	cp -a * /tmp/${ARGS}
	git show ${ARGS}:$(BASE).tex > /tmp/${ARGS}/$(BASE).tex
	git show ${ARGS}:$(BASE).bib > /tmp/${ARGS}/$(BASE).bib
	cd /tmp/${ARGS}/ && pdflatex $(BASE).tex &&  bibtex $(BASE)
	latexdiff-vc --git -r ${ARGS}  $(BASE).tex 
	latexdiff --exclude-textcmd="href" /tmp/${ARGS}/$(BASE).bbl $(BASE).bbl >/tmp/tmp.bbl
	mv /tmp/tmp.bbl $(BASE)-diff${ARGS}.bbl
	-pdflatex --interaction nonstopmode $(BASE)-diff${ARGS}.tex
	-pdflatex --interaction nonstopmode $(BASE)-diff${ARGS}.tex
	-pdflatex --interaction nonstopmode $(BASE)-diff${ARGS}.tex
	-rm $(BASE)-diff${ARGS}.aux 
	-rm $(BASE)-diff${ARGS}.log
	-rm $(BASE)-diff${ARGS}.blg
	-rm $(BASE)-diff${ARGS}.bbl
	-rm $(BASE)-diff${ARGS}.spl

## untested; don't use
distbib:
	cat $(BASE).tex | perl -e 'while(<>){if (/(\\bibliography{.+?})/) {print "\%\%$1\n"; print "\\bibliography{$(BASE)}\n"} else {print;} }' > $(BASE)-new.tex

## svn propset svn:keywords ’Id Author Date Rev URL’ *.tex


==> sections/2-Distinguish.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Update of the Plan for Exploitation and Dissemination of Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage
\section{Orchestration of Le-TSFM}
\label{sec:design}
\letsfm{} is a transformer-based, multi-expert, decoder-only model with parameters of 150 million, pre-trained on extensive real-world data from 12 business domains and synthetic data from a diffusion-based data augmentation model, and offers robust generalization capability and adaptivity across various business scenarios.


\subsection{Model Framework}
\zhengtodo{Add the architecture/framework of our time series foundation model}

\todo{Learn from Team: why do we build a decoder-only time series foundation modal? How about other types, recurrent neural network, convolution neural network, transformer-based network, etc.}



\subsection{Pre-training} 
\zhengtodo{Please add some brief descriptions and illustrations.}

\subsubsection{Tokenization} 

\subsubsection{Pre-Training}
settings, parameter searching and hardware, training times, implementation approaches, prediction approaches: rolling, long time. ? 

performance of training

\subsubsection{Hyperparameter Search}

\subsection{Benchmark?}

To summarise, \letsfm{} is a building block for diverse tasks and in the following section, we will introduce the exact features that empower its adaptiveness across business domains. 


==> sections/abbreviations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% List of Abbreviations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\clearpage
\section*{List of Abbreviations}
\label{sec:abbreviations}

\begin{acronym}[ABCDEF]
	\acro{DMP}{Data Management Plan}
	\acro{DoA}{Description of Action}
	\acro{DoI}{Digital Object Identifier}
	\acro{EU}{European Union}
	\acro{GA}{Grant Agreement}
	\acro{OA}{Open Access}
	\acro{RP}{Reporting Period}
	\acro{PM}{Person Month}
	\acro{WP}{Work Package}
\end{acronym}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
